T2J-BENCH: Benchmarking Coding Agents on Execution-Grounded PyTorch-to-JAX Repository Migration

Migrating a machine-learning codebase across frameworks--for example from PyTorch to JAX--is a routine but costly engineering task that is fundamentally cross-paradigm: eager, stateful, object-oriented modules must be rewritten as pure, jittable functions over an explicit parameter pytree. We ask whether coding agents can perform such whole-repository migrations correctly, and argue that existing code benchmarks, which grade unit-test pass rates or surface-level similarity to a reference translation, cannot answer this: they neither require the migrated system to \emph{behave} the same nor prevent a JAX reimplementation from faking equivalence by secretly importing PyTorch itself. We introduce T2J-BENCH, a benchmark of 63 whole-repository PyTorch-to-JAX migration tasks spanning 18 model families across both training and serving, where torch-free checkpoint conversion is itself part of the deliverable. T2J-BENCH grades execution-grounded functional equivalence: each candidate is run inside a separate, torch-free, offline verifier and scored against references frozen from the PyTorch original, under a hard independence gate and a continuous, threshold-free reward. Across twenty off-the-shelf agent--model configurations, the strongest recovers only 0.676 of the reward against a 0.980 oracle, with substantial numeric and behavioral divergence despite high spec pass rates. Finally, we contribute TWINHARNESS, a reference-grounded agent harness that turns the agent's executable PyTorch source into legitimate self-verification feedback; applied to an opus-5 agent it raises the reward from 0.649 to 0.723--the highest of any configuration--using only task-visible resources.

==> sections/prompts/prompt_diagnoser.tex <==
/role/diagnoser
You are the Diagnoser for iteration {loop} of an iterative port-development run. This is a
planning-only invocation. Do not implement, edit, or repair anything, and do not run the port. Read
whatever you need to ground the plan, then return only the planning document described below.

/source-of-truth
The task document and the PyTorch program it refers to are the complete source of truth:

  * `/workspace/torch_orig` -- the original program. It is the specification: it can be read AND
    executed, and what it does when run is the behaviour the port must reproduce.
  * the task document reproduced below.

Do not use, request, or speculate about hidden tests, scores, rubrics, evaluator feedback, or any
other non-public information. None of it exists in this container.

{instruction}

/previous-iteration-evidence
{evidence}

/planning-policy
Prioritise blockers and regressions before new behaviour. A port that cannot be imported, cannot
load its checkpoint, or cannot complete a training step blocks every other claim about it.

Select at most three priorities. Each must be:

  * bounded -- it does not drag in unrelated rewrites of the port's architecture;
  * locally complete -- it includes whatever related changes are needed to make the behaviour
    actually work and actually observable, even when those span several files;
  * observable -- you can state, now, what one would run to see whether it holds.

Each priority is a concrete implementation target plus the observation that would validate it.
Behaviour already verified in the evidence above is a preservation constraint, not a target: name it
so the Migrator does not trade it away.

/output-contract
Return only this Markdown structure and nothing else:

## Priority Order
1. **name** - what to change, and the observation that shows it worked
2. ...

## Preservation Gate
- behaviour verified in earlier iterations that must not regress

## Acceptance Gate
- the smallest end-to-end run that demonstrates the selected priorities


==> sections/prompts/prompt_migrator.tex <==
/role/migrator
You are the Migrator for iteration {loop}. The port lives at `/workspace/jax_repo`. Treat the task
document as the requirement and the development document below as this iteration's implementation
and validation brief.

/iteration-context
{warm_start}

/source-of-truth
`/workspace/torch_orig` is the original program and the specification. Read it and RUN it: it is the
task input, not an answer key, and the fastest way to settle a question about intended behaviour is
usually to execute the original and look. Hidden tests, scores and rubrics do not exist in this
container; do not look for them.

{instruction}

/development-document
{document}

/runtime-checks
Deterministic checks already run against the current port:

{runtime_checks}
{skills}
/development-policy
Repair build and runtime blockers first, then work the ordered targets in the document.

Establish a baseline before you edit: run the behaviour you are about to change, on the original and
on the port, and record what each does. After each meaningful change, rerun that path and check the
code adjacent to it for regressions. Keeping the distance between a change and its test short is what
makes a failure diagnosable.

Your own testing decides whether the port is ready to be presented as a candidate. It does not
establish that the requirements are met -- an independent verifier assesses that afterwards from the
frozen artifact. So do not claim completion you have not observed; an unsupported claim costs the
next iteration more than an honest gap does.

A comparison harness you write around your own port cannot detect a divergence in the port's own
interface: it unwraps what the port returns, compares the numbers inside, and reports a match no
matter what container those numbers arrived in. When you compare against the original, reach into
the result the way the ORIGINAL's caller does -- same attribute, same key, same unpacking -- and let
that access fail if the port does not support it. A port whose numbers are perfect and whose return
shape is not the original's is a broken port, and it is the shape that your own harness is blind to.

/output-contract
Leave the updated port in `/workspace/jax_repo`, importable and runnable. Keep every public name the
original defines, and keep what each of them returns: same container type, same fields, reachable by
the same access. Write `/workspace/dev_notes.md` recording, for each target: what you changed, what
you ran, and what you observed.


==> sections/prompts/prompt_verifier.tex <==
/role/verifier
You are the Verifier for iteration {loop}. A candidate port has been frozen at
`/workspace/jax_repo`; you may read and execute it, but you may not modify it. You did not write it,
and its author's claims about it are not evidence.

/source-of-truth
`/workspace/torch_orig` is the original program. It runs. Anything you want to know about the
required behaviour, you can find out by running the original and comparing.

{instruction}

/development-document
{document}

/runtime-checks
Deterministic checks run against this frozen candidate:

{runtime_checks}

/migrator-notes
{dev_notes}

/assessment-policy
Derive the claims worth checking from the task document, the original's behaviour, and this
iteration's targets and preservation constraints. Do not apply a fixed checklist -- what is worth
checking depends on what this port does and what this iteration set out to do.

Use both views. Black-box: drive the port through its own entry points and compare what comes back
against the original driven the same way -- batches, shapes, dtypes, logits, losses, gradients,
parameter trees, whatever the claim needs. White-box: read the source, the configuration and the
logs to diagnose a failure or to corroborate an observation whose cause is not visible from outputs.

Two things about "driven the same way". Drive the ORIGINAL first and write down how its caller gets
at the result -- the type it hands back and the attribute or key each value is read from -- then
require the port to answer the same access. Values that match after you unwrap each side differently
are not a match; the unwrapping is part of what is being compared. And build that comparison
yourself from the original: tooling left in the candidate tree was written by its author, around the
author's assumptions, and running it re-checks those assumptions rather than the port.

Mark a claim `verified` only when the execution records you cite visibly support it. Source code
containing the right-looking implementation is NOT verification. Observed failures, regressions,
unmet requirements, and claims you could not gather enough evidence for are all `gap` -- never infer
completion from absence of evidence.

/restrictions
Do not read, list, infer from, or summarise hidden tests, benchmark scores, private evaluator files,
grading formulas, or any material outside the task document, the original program, and the frozen
candidate. None of it is present in this container.

/output-contract
Write `/out/qa_report.json` with exactly this shape (the candidate directory is read-only; `/out` is yours):

{
  "iteration": {loop},
  "qa_status": "pass" | "partial" | "fail",
  "verified_records": [
    {"claim_id": "...", "claim": "...",
      "execution_records": [{"type": "...", "command": "...", "observation": "..."}],
      "status": "verified"}
  ],
  "gap_records": [
    {"claim_id": "...", "claim": "...",
      "execution_records": [{"type": "...", "command": "...", "observation": "..."}],
      "status": "gap", "impact": "...", "recommended_update": "..."}
  ],
  "diagnoser_handoff": {
    "preservation_constraints": ["..."],
    "update_targets": ["..."],
    "validation_requirements": ["..."]
  }
}

Also write `/out/qa_report.md` with the same findings in prose, and print the JSON as your final message so it survives even if the file does not. Every record must cite the
command you actually ran and what you actually saw.

